Revisiting Beamforming Design for Stable Millimeter-Wave Communications Under Blockages

This paper investigates robust analog beamforming for millimeter-wave (mmWave) communications under stochastic path blockages using multi-panel arrays. Conventional designs concentrate beams on the line-of-sight (LoS) path to maximize array gain, but this approach is highly vulnerable to sudden disconnections when the LoS path is blocked. To overcome this limitation, we propose a multi-beam design that exploits both LoS and non-line-of-sight (NLoS) paths for stable communications. The major contribution of this work is to establish a theoretical foundation for multi-beam design, where closed-form expressions for the cumulative distribution function (CDF) and outage probability of the spectral efficiency (SE) are derived. To design the optimal multi-beam based on the derived outage probability, we formulate a panel allocation problem to determine the assignment of panels to specific paths. The optimization problem can be solved by two algorithms based on brute-force search. Through computer simulations, the validity of the theoretical analysis for multi-beam design is confirmed, and the proposed algorithms substantially reduce the outage probability while maintaining average SE performance, thereby achieving stable communication.

==> titlepage.tex <==
% Titles are generally capitalized except for words such as a, an, and, as,
% at, but, by, for, in, nor, of, on, or, the, to and up, which are usually
% not capitalized unless they are the first or last word of the title.
% Linebreaks \\ can be used within to get better formatting as desired.
% Do not put math or special symbols in the title.
\title{Progress Report}


% author names and affiliations
% use a multiple column layout for up to three different
% affiliations
\author{\IEEEauthorblockN{Kanta Terui$^\ast$}
\IEEEauthorblockA{$^\ast$Advanced Wireless \& Communication Research Center (AWCC), 
The University of Electro-Communications,\\
1-5-1 Chofugaoka, Chofu, Tokyo 182-8585, Japan\\
Email: $^\ast$terui@awcc.uec.ac.jp}
}
% \author{\IEEEauthorblockN{Michael Shell}
% \IEEEauthorblockA{School of Electrical and\\Computer Engineering\\
% Georgia Institute of Technology\\
% Atlanta, Georgia 30332--0250\\
% Email: http://www.michaelshell.org/contact.html}
% \and
% \IEEEauthorblockN{Homer Simpson}
% \IEEEauthorblockA{Twentieth Century Fox\\
% Springfield, USA\\
% Email: homer@thesimpsons.com}
% \and
% \IEEEauthorblockN{James Kirk\\ and Montgomery Scott}
% \IEEEauthorblockA{Starfleet Academy\\
% San Francisco, California 96678--2391\\
% Telephone: (800) 555--1212\\
% Fax: (888) 555--1212}}

% conference papers do not typically use \thanks and this command
% is locked out in conference mode. If really needed, such as for
% the acknowledgment of grants, issue a \IEEEoverridecommandlockouts
% after \documentclass

% for over three affiliations, or if they all won't fit within the width
% of the page, use this alternative format:
% 
%\author{\IEEEauthorblockN{Michael Shell\IEEEauthorrefmark{1},
%Homer Simpson\IEEEauthorrefmark{2},
%James Kirk\IEEEauthorrefmark{3}, 
%Montgomery Scott\IEEEauthorrefmark{3} and
%Eldon Tyrell\IEEEauthorrefmark{4}}
%\IEEEauthorblockA{\IEEEauthorrefmark{1}School of Electrical and Computer Engineering\\
%Georgia Institute of Technology,
%Atlanta, Georgia 30332--0250\\ Email: see http://www.michaelshell.org/contact.html}
%\IEEEauthorblockA{\IEEEauthorrefmark{2}Twentieth Century Fox, Springfield, USA\\
%Email: homer@thesimpsons.com}
%\IEEEauthorblockA{\IEEEauthorrefmark{3}Starfleet Academy, San Francisco, California 96678-2391\\
%Telephone: (800) 555--1212, Fax: (888) 555--1212}
%\IEEEauthorblockA{\IEEEauthorrefmark{4}Tyrell Inc., 123 Replicant Street, Los Angeles, California 90210--4321}}



